Additive Networks of Chen-Fliess Series: Local Convergence and Relative Degree

Given an additive network of input-output systems where each node of the network is modeled by a locally convergent Chen-Fliess series, two basic properties of the network are established. First, it is shown that every input-output map between a given pair of nodes has a locally convergent Chen-Fliess series representation. Second, sufficient conditions are given under which the input-output map between a pair of nodes has a well defined relative degree as defined by its generating series. This analysis leads to the conclusion that this relative degree property is generic in a certain sense.

==> initial submission arxiv version/CSSPreamble.tex <==
%%% ============================================================================================================= %%%
%%%                                  The lastest updated date: November 11th, 2004                                    %%%
%%% ============================================================================================================= %%%
%%% Update Log: 11/16/2004, add the \RomanNumber and \romannumber for capital and small Roman numbers
%%%                         add \rb for table raising box
%%% Update Log: 05/08/2004, add the matlab and simulink definition in the end for reference
%%% Update Log: 04/26/2004, add the math operator ``dist'', update the definition for theorem-like enviroments
%%% Update Log: 03/04/2004, use package 'upgreek' for constants, e.g., $\uppi$ = 3.1415926.... (ISO standard)
%%% Update Log: 09/12/2004, update for solving the conflicts between amsthm and cssconf
%%% ============================================================================================================= %%%

\usepackage{latexsym, amssymb, amsmath}
\usepackage[dvips]{graphicx} % added for inserting the pictures
%% \usepackage[dvips]{color}
%% \usepackage{amsthm}
%% \usepackage{amscd}% amscd for "commutative diagram"
\usepackage{enumerate}
%% \usepackage{url}
%\usepackage{upref} % make all ref's are upright fonttype, no use in this paper % zzz: removed by Dr. Gray and Dr. Gonzalez
%% \usepackage{upgreek} % use upright greek to represent constant values, i.e., $\uppi$ = 3.14, ...
\usepackage{flushend} % align at the last lines of every page
\usepackage{mathrsfs} % added by Hong for Script Capital Letters by using "$\mathscr{}$"
%% \usepackage{easybmat} % A simple package for writing block matrices with equal column widths or equal rows heights or both, with various kinds of rules between rows and columns.
%% \usepackage{txfonts}%, pxfonts
%% \usepackage{euscript} %, amsfonts}
%% \usepackage{times}
%% \usepackage{color}
\usepackage{stfloats}
%% \usepackage{float}
%% Packages added by Dr. Gonzalez
%\usepackage{indentfirst}    %Automatically indents the beginning of the paragraph following a Latex section
\usepackage{cite}
%%% ============================================================================================================= %%%

% Hong's setting for figures for this paper
%\setlength{\textfloatsep}{.3em}
%\setlength{\intextsep}{.5em}

% Reduce Space Between Paragraphs
%\setlength{\parskip}{1.5ex} %plus 1pt minus 1pt}

% Reduce Space Above and Below Equations
%\setlength{\jot}{-0.7pt} % eqnarray extra space
%\setlength{\abovedisplayskip}{-1pt}% plus 1pt minus 1pt} % extra space above eqn
%\setlength{\abovedisplayshortskip}{-1pt}% plus 1pt minus 1pt} % extra space above eqn
%\setlength{\belowdisplayskip}{-1pt}% plus 1pt minus 1pt} % extra space below eqn
%\setlength{\belowdisplayshortskip}{-1pt}% plus 1pt minus 1pt} % extra space below eqn
%\setlength{\topsep}{0.2pt}

% Insert Breaks Between a Long Formula
\allowdisplaybreaks[3] % added by Hong for allowing page breaks among a large formula


%%% ============================================================================================================= %%%
% new theorems environment
%\swapnumbers
%% \theoremstyle{plain} % default
\newtheorem{prop}{Proposition} % [section]
\newtheorem{proposition}[prop]{Proposition} % [section]
\newtheorem{lem}{Lemma} % [section]
\newtheorem{lemma}[lem]{Lemma} % [section]
\newtheorem{thm}{Theorem} % [section]
\newtheorem{theorem}[thm]{Theorem} % [section]
\newtheorem{cor}{Corollary} % [section]
\newtheorem{corollary}[cor]{Corollary} % [section]
%\newtheorem{exer}{Exercise}[section]
%\newtheorem{test}{Test}[section]

%% \theoremstyle{definition}
\newtheorem{defn}{Definition} % [section]
\newtheorem{defi}[defn]{Definition} % [section]
\newtheorem{definition}[defn]{Definition} % [section]
\newtheorem{conj}{Conjecture} % [section]
\newtheorem{exmp}{Example} % [section]
\newtheorem{example}[exmp]{Example} % [section]
\newtheorem{exam}[exmp]{Example} % [section]
\newtheorem{exam*}{Example}

%% \theoremstyle{remark}
%% \newtheorem*{rmk}{Remark}
%% \newtheorem*{remark}{Remark}
% %\newtheorem*{note}{Note}
% \newtheorem{case}{Case}

% \newtheoremstyle{model}% name
%   {3pt}%      Space above, empty = `usual value'
%   {3pt}%      Space below
%   {\itshape}% Body font
%   {}%         Indent amount (empty = no indent, \parindent = para indent)
%   {\textnormal}% Thm head font
%   {.}%        Punctuation after thm head
%   {.5em}%     Space after thm head: " " = normal interword space;
%         %       \newline = linebreak
%   {}% Thm head spec
%\renewcommand {\thmhead}[3]{\thmname{#1}\thmnumber{#2}\thmnote{\textnormal{[\emph{#3}]}}}

% \theoremstyle{model}
% \newtheorem*{mdl}{Rollback Interference Model}


%%% ============================================================================================================= %%%
% Generates a bibliography with 'References' centered above the column, changed by Hong
\def\custombibliography#1{
 \normalsize
% The part was commented by Hong
% \begin{center}
% {\Large \bf{References}}
% \end{center}
\section*{\centering References}
 \list
 {[\arabic{enumi}]}{\settowidth\labelwidth{[#1]}\leftmargin\labelwidth
 \setlength{\itemsep}{.1em}
 \advance\leftmargin\labelsep
 \usecounter{enumi}}
 \def\newblock{\hskip .11em plus .33em minus -.07em}
 \sloppy
 \sfcode`\.=1000\relax}
\let\endthebibliography=\endlist


%%% ============================================================================================================= %%%
% Gray's Abbreviations
\def\L2{{\cal L}_2}
\def\begar{\begin{array}}
\def\endar{\end{array}}
\def\begce{\begin{center}}
\def\endce{\end{center}}
\def\begco{\begin{cor}}
\def\endco{\end{cor}}
\def\begde{\begin{defn}}
\def\endde{\end{defn}}
\def\begdes{\begin{description}}
\def\enddes{\end{description}}
\def\begdi{\begin{displaymath}}
\def\enddi{\end{displaymath}}
\def\begdis{\begin{eqnarray*}}
\def\enddis{\end{eqnarray*}}
\def\begen{\begin{enumerate}}
\def\enden{\end{enumerate}}
\def\begeq{\begin{equation}}
\def\endeq{\end{equation}}
\def\begeqa{\begin{eqnarray}}
\def\endeqa{\end{eqnarray}}
\def\begex{\begin{exmp}}
\def\endex{\end{exmp}}
\def\begfig{\begin{fig}}
\def\endfig{\end{fig}}
\def\begit{\begin{itemize}}
\def\endit{\end{itemize}}
\def\begle{\begin{lem}}
\def\endle{\end{lem}}
\def\begpro{\begin{prop}} % added by Hong
\def\endpro{\end{prop}} % added by Hong
\def\begth{\begin{thm}}
\def\endth{\end{thm}}
\def\begre{\noindent{\bf Remark}:\ } % changed by Hong
\def\endre{\\}
\def\begres{\noindent{\bf Remarks}:\begin{enumerate}}
\def\endres{\end{enumerate} \par}
\def\begpr{\begin{proof}} % changed by Hong
\def\endpr{\end{proof}}
%\def\begpr{\noindent{\em Proof}\ : } % changed by Hong
%\def\endpr{\hspace*{0.05in}\bull\vspace*{0.15in}\\}
%\def\beglar{\left[\begin{array}}
%\def\endrar{\end{array}\right]}


%%% ============================================================================================================= %%%
% Gray's New Commands
\newcommand\bull{\vrule height .9ex width .8ex depth -.1ex } % square bullet
\newcommand\bul{$\bullet\;\;\;$}
\newcommand\re{\rm I\! R}
%\renewcommand\qed{\hfill$\Box \Box \Box$}
%\newcommand\mathbfsub#1{\hbox{\mathversion{bold}$\scriptstyle #1$}} % Stopped by Hong; Define better command \rv
%\newcommand\rref[1]{(\ref{#1})} % Stopped by Hong; Use AMS LaTeX command \eqref
\newcommand\spacebox[1]{\raisebox{-6pt}[7pt][0pt]{#1}} % puts extra space around items in a table
\newcommand\cdcout[1]{} % reduce it to 6 pages
%\newcommand\cdcout[1]{#1} % restores the CDC 7 page version


%%% ============================================================================================================= %%%
% Hong's Abbreviations for Left and Right Delimiters
\newcommand{\Lb}{\left [}          % Left bracket
\newcommand{\Rb}{\right ]}         % Right bracket
\newcommand{\LB}{\left \{}         % Left brace
\newcommand{\RB}{\right \}}        % Right brace
\newcommand{\Ld}{\left .}          % Left default
\newcommand{\Rd}{\right .}         % Right default
\newcommand{\Lp}{\left (}          % Left parenthese
\newcommand{\Rp}{\right )}         % Right parenthese
\newcommand{\Lv}{\left |}          % Left vertical line
\newcommand{\Rv}{\right |}         % Right vertical line
\newcommand{\LV}{\left \|}         % Left vertical double line
\newcommand{\RV}{\right \|}        % Right vertical double line


%%% ============================================================================================================= %%%
% Hong's New Commands and Declarations for Linear Algebra and Matrix Analysis
\DeclareMathOperator{\trace}{tr}   % Define a matrix' trace operator, sometimes
\DeclareMathOperator{\diag}{diag}  % Define the diagonal matrix operator
\DeclareMathOperator{\rank}{rank}  % Define the rank operator of a matrix
\DeclareMathOperator{\vect}{vec}   % Define the function to reshape a matrix into a vector column-wise.
% \DeclareMathOperator{\col}{col}    % Define the column operator, e.g., $cy = \col \LB y_i, \dots, y_n \RB$
\newcommand{\T}{^\mathrm{T}}       % Transposition operator of the matrix or vector
\newcommand{\h}{^\mathrm{H}}       % Hermitian Transposition of a matrix or vector


%%% ============================================================================================================= %%%
% Hong's New Commands and Declarations for Random Variables, Probability and Stochastic Process
\newcommand{\rv}[1]{\boldsymbol{#1}} % Use italic boldface to indicate the Random Variables
\DeclareMathOperator{\Var}{Var}      % Operator for variance of a RV
\DeclareMathOperator{\Cov}{Cov}      % Operator for covariance of a RV
\DeclareMathOperator*{\Lim}{l.i.m.}  % Operator for convergence in the MS sense

%%% ============================================================================================================= %%%
% Hong's New Commands and Declarations for Mathematical Analysis and Other Areas
\DeclareMathOperator{\sgn}{sgn}      % Operator for sign function
\DeclareMathOperator*{\argmax}{\arg\max}
\DeclareMathOperator{\dist}{dist}

%%% ============================================================================================================= %%%
%% New Commands for Sets or Spaces
\newcommand{\N}{\mathbb N} % for the set of natural
\newcommand{\C}{\mathbb C} % for the set of complex
\newcommand{\Q}{\mathbb Q} % for the set of rational
\newcommand{\R}{\mathbb R} % for the set of real
\newcommand{\Z}{\mathbb Z} % for the set of integer

%%% ============================================================================================================= %%%
% International Typesetting Standards
\newcommand{\me}{\mathrm{e}} % for math e
\newcommand{\mi}{\mathrm{i}} % for math i
\newcommand{\mj}{\mathrm{j}} % added by Hong for engineering j
\newcommand{\dif}{\,\mathrm{d}}% for differential

%%% ============================================================================================================= %%%
%% Hong's abbreviations of sets or spaces for this paper
\newcommand{\MRn}{\mathbb M(\R^{n})}
\newcommand{\Hn}{\mathbb H^n}
\newcommand{\Hnp}{\mathbb H^{n+}}
\newcommand{\BHn}{\mathbb B(\Hn)}

%%% ============================================================================================================= %%%
%% Hong's other settings just for this paper
%% \renewcommand{\labelenumi}{\textup{(\alph{enumi})}}
%% \setlength{\topsep}{-1pt}
%%\setlength{\itemsep}{-5pt}

%%% ============================================================================================================= %%%
%% Hong's other commands
\newcommand{\matlab}{\textsc{MATLAB}\textsuperscript{\textregistered}} % for the mathworks MATLAB registered product
\newcommand{\simulink}{Simulink\textsuperscript{\textregistered}} % for the mathworks Simulink registered product

%%% ============================================================================================================= %%%
%% Hong's Capital/Small Roman Numbers
\newcommand{\RomanNumber}[1]{\uppercase\expandafter{\romannumeral #1}}
\newcommand{\romannumber}[1]{\lowercase\expandafter{\romannumeral #1}}

%%% ============================================================================================================= %%%
%% Hong's Fonts definitions

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

%% Table Raising box
\newcommand{\rb}[1]{\raisebox{1.5ex}[0pt]{#1}}

%%% ============================================================================================================= %%%
%% Dr. Gonzalez's Group definitions
\def\1{\rv 1} %Indicator
\def\I{{\mathcal I}}    %Index set
\def\E{{\mathbb E}}    %PDP state space
\def\bE{{\mathcal E}}    %Borel set
\def\x{{\rv\chi}}    %hybrid PDP state
\def\B{{\mathcal B}}    %Index set




%\renewcommand{\baselinestretch}{0.9}


==> initial submission arxiv version/abbreviations.tex <==

% Master List of Latex Abbreviations

% Color Abbreviations
%
\def\bluetext#1{\textcolor[rgb]{0.00,0.00,1.00}{#1}}
\def\blacktext#1{\textcolor[rgb]{0.00,0.00,0.00}{#1}}
\def\redtext#1{\textcolor[rgb]{0.98,0.00,0.00}{#1}}
\def\yellowtext#1{\textcolor[rgb]{1.00,1.00,0.26}{#1}}
\def\whitetext#1{\textcolor[rgb]{1.00,1.00,1.0}{#1}}
\def\colornote#1{\textcolor[rgb]{1.00,0.00,0.00}{#1}}
\definecolor{Light}{gray}{0.85}

% Symbol Abbreviations

% Aa
\def\adj{{\rm adj}}
\def\abs#1{\left\vert #1 \right\vert}
%
\def\allcommutingpoly{\mbox{$\re[X]$}}
%--------------------------------------------------------------------------
% Want to make these obsolete to avoid conflict in second group
%\def\allcommutingseries{\mbox{$\re\, [[\tilde{X}]]$}}
%\def\allcommutingseriesell{\mbox{$\re^{\ell}\, [[\tilde{X}]]$}}
%\def\allcommutingseriesm{\mbox{$\re^{m}\, [[\tilde{X}]]$}}
%--------------------------------------------------------------------------
% These are my standard definitions
\def\allcommutingseries{\mbox{$\re\, [[X]]$}}
\def\allcommutingseriesell{\mbox{$\re^{\ell}\, [[X]]$}}
\def\allcommutingseriesellGC{\mbox{$\re^{\ell}_{GC}\, [[X]]$}}
\def\allcommutingseriesellLC{\mbox{$\re^{\ell}_{LC}\, [[X]]$}}
\def\allcommutingseriestildeellGC{\mbox{$\re_{GC}^{\tilde{\ell}}\, [[X]]$}}
\def\allcommutingseriestildem{\mbox{$\re^{\tilde{m}}\, [[X]]$}}
\def\allcommutingseriestildemGC{\mbox{$\re_{GC}^{\tilde{m}}\, [[X]]$}}
\def\allcommutingseriestildemLC{\mbox{$\re_{LC}^{\tilde{m}}\, [[X]]$}}
\def\allcommutingseriestildeX{\mbox{$\re\, [[\tilde{X}]]$}}
\def\allcommutingseriestildeXell{\mbox{$\re^{\ell}\, [[\tilde{X}]]$}}
\def\allcommutingseriestildeXellLC{\mbox{$\re_{LC}^{\ell}\, [[\tilde{X}]]$}}
\def\allcommutingseriestildeXellGC{\mbox{$\re_{GC}^{\ell}\, [[\tilde{X}]]$}}
\def\allcommutingseriestildeXtildeell{\mbox{$\re^{\tilde{\ell}}\, [[\tilde{X}]]$}}
\def\allcommutingseriestildeXtildeellLC{\mbox{$\re_{LC}^{\tilde{\ell}}\, [[\tilde{X}]]$}}
\def\allcommutingseriestildeXtildeellGC{\mbox{$\re_{GC}^{\tilde{\ell}}\, [[\tilde{X}]]$}}
\def\allcommutingseriestildeXtildemLC{\mbox{$\re_{LC}^{\tilde{m}}\, [[\tilde{X}]]$}}
\def\allcommutingseriestildeXtildemGC{\mbox{$\re_{GC}^{\tilde{m}}\, [[\tilde{X}]]$}}
%---------------------------------------------------------------------------------
% These should also become obsolete.
%\def\allcommutingseriesX{\mbox{$\re\, [[X]]$}}
%\def\allcommutingseriesXm{\mbox{$\re^m\, [[X]]$}}
%\def\allcommutingseriesXell{\mbox{$\re^{\ell}\, [[X]]$}}
%\def\allcommutingseriesXOell{\mbox{$\re^{\ell}\, [[X_0]]$}}
%\def\allcommutingseriesXtildeellLC{\mbox{$\re_{LC}^{\tilde{\ell}}\, [[X]]$}}
%\def\allcommutingseriesXtildeellGC{\mbox{$\re_{GC}^{\tilde{\ell}}\, [[X]]$}}
%\def\allcommutingseriesXtildemLC{\mbox{$\re_{LC}^{\tilde{m}}\, [[X]]$}}
%\def\allcommutingseriesXtildemGC{\mbox{$\re_{GC}^{\tilde{m}}\, [[X]]$}}
%
\def\allpoly{\mbox{$\re\langle X \rangle$}}
\def\allpolyell{\mbox{$\re^{\ell}\langle X \rangle$}}
%\def\allpolyx0{\mbox{$\re[[ x_0 ]]$}} % This convention is obsolete
\def\allpolyx0degn{\mbox{$P_n$}}
\def\allpolyXO{\mbox{$\re [X_0]$}}
\def\allpolyXOm{\mbox{$\re^m [X_0]$}}
\def\allpolyXW{\mbox{$\re\langle XW \rangle$}}
%\def\allpolyI{\mbox{$\re\langle I \rangle$}} % This convention is obsolete
%
\def\allseries{\mbox{$\re\langle\langle X \rangle\rangle$}}
\def\allseriesdelta{\mbox{$\re\langle\langle X_\delta \rangle\rangle$}}
\def\allseriesdeltam{\mbox{$\re^m\langle\langle X_\delta \rangle\rangle$}}
\def\allseriesdeltaL{\mbox{$\re_{L}\langle\langle X_\delta \rangle\rangle$}}
\def\allseriesdeltaLC{\mbox{$\re_{LC}\langle\langle X_\delta \rangle\rangle$}}
\def\allseriesdeltamL{\mbox{$\re^m_{L}\langle\langle X_\delta \rangle\rangle$}}
\def\allseriesdeltamLC{\mbox{$\re^m_{LC}\langle\langle X_\delta \rangle\rangle$}}
\def\allseriesell{\mbox{$\re^{\ell} \langle\langle X \rangle\rangle$}}
\def\allseriesGC{\mbox{$\re_{GC}\langle\langle X \rangle\rangle$}}
\def\allseriesLC{\mbox{$\re_{LC}\langle\langle X \rangle\rangle$}}
\def\allseriesm{\mbox{$\re^m\langle\langle X \rangle\rangle$}}
\def\allseriesmtimesm{\mbox{$\re^{m\times m}\langle\langle X \rangle\rangle$}}
\def\allseriesmDF{\mbox{$\re^m\langle\langle \tilde{X} \rangle\rangle$}}
\def\allseriesmGC{\mbox{$\re^{m}_{GC}\langle\langle X \rangle\rangle$}}
\def\allseriesmLC{\mbox{$\re^{m}_{LC}\langle\langle X \rangle\rangle$}}
\def\allseriesmLCDF{\mbox{$\re^{m}_{LC}\langle\langle \tilde{X} \rangle\rangle$}}
\def\allseriesnLC{\mbox{$\re^{n}_{LC}\langle\langle X \rangle\rangle$}}
\def\allseriesnGC{\mbox{$\re^{n}_{GC}\langle\langle X \rangle\rangle$}}
\def\allseriesn{\mbox{$\re^n\langle\langle X \rangle\rangle$}}
\def\allseriesntimesn{\mbox{$\re^{n\times n}\langle\langle X \rangle\rangle$}}
\def\allseriesSLC{\mbox{$\re_{LC}\langle\langle S \rangle\rangle$}}
\def\allZseries{\mbox{$\mathbb{Z}\langle\langle X \rangle\rangle$}}
%
\def\allseriestildeell{\mbox{$\re^{\tilde{\ell}} \langle\langle X \rangle\rangle$}}
\def\allseriestildeellGC{\mbox{$\re^{\tilde{\ell}}_{GC} \langle\langle X \rangle\rangle$}}
\def\allseriestildeellLC{\mbox{$\re^{\tilde{\ell}}_{LC} \langle\langle X \rangle\rangle$}}
\def\allseriestildem{\mbox{$\re^{\tilde{m}} \langle\langle X \rangle\rangle$}}
\def\allseriestildemGC{\mbox{$\re^{\tilde{m}}_{GC} \langle\langle X \rangle\rangle$}}
\def\allseriestildemLC{\mbox{$\re^{\tilde{m}}_{LC} \langle\langle X \rangle\rangle$}}
\def\allseriestildeX{\mbox{$\re \langle\langle \tilde{X} \rangle\rangle$}}
\def\allseriestildeXell{\mbox{$\re^\ell \langle\langle \tilde{X} \rangle\rangle$}}
\def\allseriestildeXLC{\mbox{$\re^\ell_{LC} \langle\langle \tilde{X} \rangle\rangle$}}
\def\allseriestildeXtildeell{\mbox{$\re^{\tilde{\ell}} \langle\langle \tilde{X} \rangle\rangle$}}
\def\allseriestildeXtildeellGC{\mbox{$\re^{\tilde{\ell}}_{GC} \langle\langle \tilde{X} \rangle\rangle$}}
\def\allseriestildeXtildeellLC{\mbox{$\re^{\tilde{\ell}}_{LC} \langle\langle \tilde{X} \rangle\rangle$}}
%
\def\allseriesellLC{\mbox{$\re^{\ell}_{LC}\langle\langle X \rangle\rangle$}}
\def\allseriesellGC{\mbox{$\re^{\ell}_{GC}\langle\langle X \rangle\rangle$}}
\def\allseriestwo{\mbox{$\re^{2}\langle\langle X \rangle\rangle$}}
\def\allseriestwoLC{\mbox{$\re^{2}_{LC}\langle\langle X \rangle\rangle$}}
% These are obsolete
%\def\allseriesI{\mbox{$\re\langle\langle I \rangle\rangle$}}
%\def\allseriesILC{\mbox{$\re_{LC}\langle\langle I \rangle\rangle$}}
%\def\allseriesIm{\mbox{$\re^m\langle\langle I \rangle\rangle$}}
%\def\allseriesImLC{\mbox{$\re^m_{LC}\langle\langle I \rangle\rangle$}}
%\def\allseriesIell{\mbox{$\re^{\ell}\langle\langle I \rangle\rangle$}}
%\def\allseriesIellLC{\mbox{$\re^{\ell}_{LC}\langle\langle I \rangle\rangle$}}
\def\allseriesx{\mbox{$\re[[x]]$}}
\def\allseriesXO{\mbox{$\re [[ X_0 ]]$}}
\def\allseriesXOm{\mbox{$\re^m [[ X_0 ]]$}} % use oh since zero is not allowed
\def\allseriesXOmLC{\mbox{$\re^m_{LC} [[ X_0 ]]$}}
\def\allseriesXOell{\mbox{$\re^{\ell} [[ X_0 ]]$}}
\def\allseriesXOellLC{\mbox{$\re^{\ell}_{LC} [[ X_0 ]]$}}
\def\allseriesXWell{\mbox{$\re^{\ell}\!\ll\!XW\!\gg$}}
\def\allseriesXW{\mbox{$\re\!\ll\!XW\!\gg$}}
\def\allseriesXWLC{\mbox{$\re_{LC}\!\ll\!XW\!\gg$}}
\def\allseriesWLC{\mbox{$\re_{LC}\!\ll\!W\!\gg$}}
\def\allseriesXWellLC{\mbox{$\re^{\ell}_{LC}\!\ll\!XW\!\gg$}}
%
\def\alltransductionsXtildeX{\mbox{$[\allseriestildeX] \langle\langle X \rangle\rangle$}}

% Bb
\def\bfem#1{{\bf \em #1}} % boldface italics
\def\borel{\mathscr{B}}
\def\borelf{\mathscr{B}_f}
\def\Bp{B_{\mathfrak{p}}}
\def\Bpm{B_{\mathfrak{p}}^m}
\def\Bq{B_{\mathfrak{q}}}
\def\Bqell{B_{\mathfrak{q}}^\ell}
\def\Bqm{B_{\mathfrak{q}}^m}
\def\bull{\rule{0.08in}{0.08in}} % square filled bullet

% Cc
\def\C{{\mathbb C}} % complex numbers (AMS symbol)
\def\Cc{{\cal C}} % class of continuous functions
\def\card{{\rm card}}
\def\charseries{{\rm char}}
\def\Chengroup{{\cal G}_C(\tilde{X})}
\def\Chenseries{{\mathcal G}_C(X)}
\def\chiup{\hbox{\raisebox{0.03in}{$\chi$}}} % slightly raised \chi symbol
\def\chiupsub{\hbox{\raisebox{0.02in}{$\scriptstyle \chi$}}} % slightly raised \chi symbol
\newcommand{\comment}[1]{} % allows one to comment out a block of text
\def\conc{{\rm cat}}
\def\convunit{\mbox{$\vartheta$}}

% Dd
\def\diag{{\rm diag}}
\def\dim{{\rm dim}}
\def\dist{{\rm dist}}
\def\down#1{{}_{{}_{#1}}}
\def\doubleone{{\rm\, l\!l}}

% Ee
\def\Endallseries{{\rm End}(\allseries)}
\def\Endallseriesm{{\rm End}(\allseriesm)}
\def\EndoA{{\rm End}(\mbox{$A$})}
%\def\EndoA{{\rm End}($A$)} % obsolete since A has \rm font
\def\eqref#1{(\ref{#1})} % parentheses around referenced equation numbers
%\def\equivf{\underset{f}{\sim}} % Does not match Chapter 1 format
\def\equivf{{\sim_f}}
\DeclareMathOperator*{\esssup}{ess\;\, sup}
\def\expdown{{\rm exp}}
\def\expup{{\rm e}}

% Ff
\def\fac{{\rm fac}}
\def\Fliessdelta{\mathscr{F}_{\delta}}
\def\FliessLC{\mathscr{F}}
\def\freegroup{{\cal F}}

% Gg
\def\GLn{GL_n(\re)}
\def\groupE{{\cal G}(E)}

% Hh
\newcommand{\hX}{\hat X}
\newcommand{\hW}{\hat W}

% Ii
\def\id{{\rm id}}
\def\im{{\rm im}}
\def\impart{{\rm Im}}
\def\innprod#1#2{\left\langle #1, #2 \right\rangle}
\def\integers{{\mathbb Z}} % integers

% Kk
\def\ker{{\rm ker}}

% Ll
\def\Lp{L_{\mathfrak{p}}}
\def\Lpm{L_{\mathfrak{p}}^m}
\def\Lpe{L_{\mathfrak{p},e}}
\def\Lpme{L^m_{\mathfrak{p},e}}
\def\Lq{L_{\mathfrak{q}}}
\def\Lqell{L_{\mathfrak{q}}^\ell}
\def\Lqm{L_{\mathfrak{q}}^m}
\def\laplace{\mathscr{L}}
\def\laplacef{\mathscr{L}_f}
\def\liead{{\rm ad}}
\def\tliead{{\rm \widetilde{ad}}}
\def\lieAd{{\rm Ad}}
\def\tlieAd{{\rm \widetilde{Ad}}}
\def\liepoly{{\mathcal L}(X)}
\def\liepolyO{{\mathcal L}_0(X)}
\def\lieseries{\widehat{\mathcal L}(X)}

% Mm
\def\Magnusgroup{{\cal G}_M(X)}
\def\Malcevgroup{\widehat{\mathcal G}(X)}
\def\MalcevgrouptildeX{\widehat{\cal G}(\tilde{X})}
\def\mbf#1{\hbox{\mathversion{bold}$#1$}} % math boldface
%\def\mbf#1{\mathbf{#1}} % special version for affine MIMO paper
\def\mbfss#1{\hbox{\scriptsize\mathversion{bold}$#1$}} % math boldface
\def\modcomp{\:\tilde{\circ}\,} % modified composition product

% Nn
\def\nat{{\mathbb N}} % natural numbers (AMS symbol)
\def\norm#1{\left\Vert#1\right\Vert}
\def\notin{{\not\in}}
\def\ns#1{{\textstyle #1}} % normalsize fonts in subscripts
\def\Null{{\rm null}}

% Oo
\def\openbull{\framebox[0.08in][c]{$\;$}} % square unfilled bullet
\def\ord{{\rm ord}}

% Pp
\def\preMalcevgroup{{\cal G}(X)}

% Qq
\def\qed{\hfill$\Box \Box \Box$}

% Rr
%\newcommand{\R}{\mathbb R} % Generates an error for this paper
\def\rank{{\rm rank}}
\def\re{{\mathbb R}} % real numbers (AMS symbol)
\def\repart{{\rm Re}}

% Ss
\def\sameau{\rule[0.017in]{0.2in}{0.012in}}
\def\sh{{\rm sh}}
\def\shlang{{\mathbb S}} % shuffle language
%\def\shuffle{{\hbox{\cyr x}}} % shuffle product using cyrillic font
\def\shuffle{{\scriptscriptstyle \;\sqcup \hspace*{-0.05cm}\sqcup\;}}
\def\shuffleXW{{{\shuffle}}}
\font\grs=eurm10 at 9pt \def\smu{{\hbox{\grs\char22}}} % use for micro...
\def\spacebox#1{\raisebox{-3pt}[5pt][7pt]{#1}} % puts extra space around items in a table
\def\spanset{{\rm span}}
\def\supp{{\rm supp}}
\def\ss#1{{\scriptstyle #1}} % fonts in subsubscripts
\def\sss#1{{\scriptscriptstyle #1}} % fonts in subsubsubscripts

% Tt
\def\Tr{{\rm Tr}}

% Uu
\font\grg=eurm10 \def\umu{{\hbox{\grg\char22}}} % upright mu.

% Vv
\def\ve{\varepsilon}
\def\vec{{\rm vec}}

% Zz
\def\Ztransform{\mathscr Z}

% Environment Abbreviations
%
% There is a Latex bug that prevents one from using shortcuts for the align
% and align* environments. The work around below for align* has a problem: it
% will not permit \displaybreak commands. So it is recommended that these
% abbreviations be avoided in general.
\def\begals{\[\begin{aligned}}
\def\endals{\end{aligned}\]}
\def\begce{\begin{center}}
\def\endce{\end{center}}
\def\begar{\begin{array}}
\def\endar{\end{array}}
\def\begeq{\begin{equation}}
\def\endeq{\end{equation}}
\def\begdi{\begin{displaymath}}
\def\enddi{\end{displaymath}}
\def\begdis{\begin{eqnarray*}}
\def\enddis{\end{eqnarray*}}
\def\begeqa{\begin{eqnarray}}
\def\endeqa{\end{eqnarray}}
\def\begdes{\begin{description}}
\def\enddes{\end{description}}
\def\begit{\begin{itemize}}
\def\endit{\end{itemize}}
\def\begen{\begin{enumerate}}
\def\enden{\end{enumerate}}
\def\beglar{\left[\begin{array}}
\def\endrar{\end{array}\right]}
\def\begle{\begin{mylemma}}
\def\endle{\end{mylemma}}
\def\begde{\begin{mydefinition}}
\def\endde{\end{mydefinition}}
\def\begth{\begin{mytheorem}}
\def\endth{\end{mytheorem}}
\def\begco{\begin{mycorollary}}
\def\endco{\end{mycorollary}}
\def\begprop{\begin{myproposition}}
\def\endprop{\end{myproposition}}
\def\begex{\begin{myexample}}
\def\endex{\hfill\openbull \end{myexample} \vspace*{0.15in}}
\def\begexer{\begin{myexercise}}
\def\endexer{\end{myexercise}}
\def\begre{\noindent{\bf Remark}:}
\def\endre{\\}
\def\begres{\noindent{\bf Remarks}:\begin{enumerate}}
\def\endres{\end{enumerate} \par}
\def\begpr{\noindent{\em Proof:}$\;\;$}
\def\endpr{\hfill\bull \vspace*{0.15in}}
\def\begtab{\begin{tabular}}
\def\endtab{\end{tabular}}
\def\rref#1{(\ref{#1})}
\def\problem#1{\vspace*{0.1in}\noindent {\bf Problem \ref{#1}}} % for the solution key

% Luis' Abbreviations for CDC 2007 insert
\def\allseriesY{\mbox{$\re\!\ll\!Y\!\gg$}}
\def\allseriesZ{\mbox{$\re\!\ll\!Z\!\gg$}}
\def\allseriestZj{\mbox{$\re\!\ll\!\tilde{Z}_j\!\gg$}}
\def\allseriesW{\mbox{$\re\!\ll\!W\!\gg$}}
\def\allseriesA{\mbox{$\re\!\ll\!A\!\gg$}}
\def\allseriesA'{\mbox{$\re\!\ll\!A'\!\gg$}}
\def\allseriesZj{\mbox{$\re\!\ll\!Z_j\!\gg$}}
\def\allseriesZbb{\mbox{$\re\!\ll\!Z\cup{\bar{\bar{Z}}}\!\gg$}}
\def\allseriesZZbZbb{\mbox{$\re\!\ll\!Z\cup\bar{Z}\cup{\bar{\bar{Z}}}\!\gg$}}
\def\allseriesrat{\mbox{$\re^{rat}\!\ll\!X\!\gg$}}
%\def\allpolyell{\mbox{$\re^{\ell}\!\!<\!\!X\!\!>$}} % conflicts with above definition
\def\allseriesXxY{\mbox{$\re\!\ll\!X\otimes Y\!\gg$}}
\def\characserie#1{{\bf{#1}^*}} % Symbol for characteristic series

